VideoSPatS: Video SPatiotemporal Splines for Disentangled Occlusion, Appearance and Motion Modeling and Editing

We present an implicit video representation for occlusions, appearance, and motion disentanglement from monocular videos, which we call Video SPatiotemporal Splines (VideoSPatS). Unlike previous methods that map time and coordinates to deformation and canonical colors, our VideoSPatS maps input coordinates into Spatial and Color Spline deformation fields $D_s$ and $D_c$, which disentangle motion and appearance in videos. With spline-based parametrization, our method naturally generates temporally consistent flow and guarantees long-term temporal consistency, which is crucial for convincing video editing. Using multiple prediction branches, our VideoSPatS model also performs layer separation between the latent video and the selected occluder. By disentangling occlusions, appearance, and motion, our method enables better spatiotemporal modeling and editing of diverse videos, including in-the-wild talking head videos with challenging occlusions, shadows, and specularities while maintaining an appropriate canonical space for editing. We also present general video modeling results on the DAVIS and CoDeF datasets, as well as our own talking head video dataset collected from open-source web videos. Extensive ablations show the combination of $D_s$ and $D_c$ under neural splines can overcome motion and appearance ambiguities, paving the way for more advanced video editing models.

==> figures/reb_dc.tex <==
\renewcommand{\arraystretch}{0.5}
\setlength{\tabcolsep}{1.0pt}
\begin{tabular}{cc|cc}
\multicolumn{2}{c}{Canonical Foreground w/ $D_c$} & \multicolumn{2}{c}{Canonical Foreground w/o $D_c$} \\
$t=0$ & $t=1$ & $t=0$ & $t=1$ \\
\includegraphics[width = 0.7in]{figures/reb_ablateDc/Dc/e160_can_occ.jpg} &
\includegraphics[width = 0.7in]{figures/reb_ablateDc/Dc/e164_can_occ.jpg} &
\includegraphics[width = 0.7in]{figures/reb_ablateDc/noDc/e160_can_occ.jpg} &
\includegraphics[width = 0.7in]{figures/reb_ablateDc/noDc/e164_can_occ.jpg} \\
\end{tabular}

==> figures/reb_edit.tex <==
\renewcommand{\arraystretch}{0.5}
\setlength{\tabcolsep}{1.2pt}
\begin{tabular}{cc|cc}
\multicolumn{2}{c}{a) CoDeF} & \multicolumn{2}{c}{b) Ours} \\
\includegraphics[width = 0.8in]{figures/reb_editing/bear/00030_codef.png} &
\includegraphics[width = 0.8in]{figures/reb_editing/bear/00081_codef.png} &
\includegraphics[width = 0.8in]{figures/reb_editing/bear/00030_ours.jpg} &
\includegraphics[width = 0.8in]{figures/reb_editing/bear/00081_ours.jpg} \\

\includegraphics[width = 0.8in]{figures/reb_editing/train/00020_codef.png} &
\includegraphics[width = 0.8in]{figures/reb_editing/train/00040_codef.png} &
\includegraphics[width = 0.8in]{figures/reb_editing/train/00020_ours.jpg} &
\includegraphics[width = 0.8in]{figures/reb_editing/train/00040_ours.jpg} \\

\end{tabular}

==> figures/reb_iters.tex <==
\renewcommand{\arraystretch}{0.5}
\setlength{\tabcolsep}{0.1pt}
\begin{tabular}{ccc}
\includegraphics[width = 0.62in]{figures/reb_iterations/e15_comp_img_10k.jpg} &
\includegraphics[width = 0.62in]{figures/reb_iterations/e40_comp_img_30k.jpg} &
\includegraphics[width = 0.62in]{figures/reb_iterations/e160_comp_img_100k.jpg} \\

10k-8.88min & 30k-27.23min & 100k-88.6min \\
30.67dB & 36.16dB & 37.21dB \\
\end{tabular}

==> figures/reb_manual.tex <==
\setlength{\tabcolsep}{0.5pt}
\begin{tabular}{cccc}
% Edited Canonical Space & Propagated & Propagated \\
\includegraphics[trim={8cm 4.5cm 8cm 4.5cm}, clip, width = 0.8in]{figures/reb_manual_edit/can_original.png} &
\includegraphics[trim={8cm 4.5cm 8cm 4.5cm}, clip, width = 0.8in]{figures/reb_manual_edit/can_edit.jpg} &
\includegraphics[width = 0.8in]{figures/reb_manual_edit/00020.jpg} &
\includegraphics[width = 0.8in]{figures/reb_manual_edit/00027.jpg}\\
\end{tabular}

==> figures/reb_revideo.tex <==
\renewcommand{\arraystretch}{0.5}
\setlength{\tabcolsep}{0.5pt}
\begin{tabular}{cc|cc|cc}
\multicolumn{2}{c}{Original} & \multicolumn{2}{c}{ReVideo} & \multicolumn{2}{c}{Ours} \\
\includegraphics[width = 0.54in]{figures/reb_revideo/frame_0000_original.png} &
\includegraphics[width = 0.54in]{figures/reb_revideo/frame_0013_original.png} &
\includegraphics[width = 0.54in]{figures/reb_revideo/frame_0000_revideo.png} &
\includegraphics[width = 0.54in]{figures/reb_revideo/frame_0013_revideo.png} &
\includegraphics[width = 0.54in]{figures/reb_revideo/00000_ours.jpg} &
\includegraphics[width = 0.54in]{figures/reb_revideo/00013_ours.jpg} \\

\end{tabular}

==> figures/sup_other_comp_backup.tex <==
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.5}
\small
\begin{tabular}{cccc}

\multicolumn{4}{c}{Neural Layered Atlasses}\\
\includegraphics[width = 1.5in]{figures/sup_other_comp_atlasses/texture_orig2_mic.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_atlasses/texture_orig2_uncle.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_atlasses/texture_orig2_green.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_atlasses/texture_orig2_hands.png} \\

\includegraphics[width = 1.5in]{figures/sup_other_comp_atlasses/texture_orig1_mic.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_atlasses/texture_orig1_uncle.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_atlasses/texture_orig1_green.png}  &
\includegraphics[width = 1.5in]{figures/sup_other_comp_atlasses/texture_orig1_hands.png} \\

\multicolumn{4}{c}{Deformable Sprites}\\
\includegraphics[width = 1.5in]{figures/sup_other_comp_sprites/Yu5Xu2qwZxo_texs_1.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_sprites/C6VbIdO42mQ_texs_1.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_sprites/MXYLgFEcagg_texs_1.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_sprites/LKJLXbiOvBg_texs_1.jpg} \\

\includegraphics[width = 1.5in]{figures/sup_other_comp_sprites/Yu5Xu2qwZxo_texs_0.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_sprites/C6VbIdO42mQ_texs_0.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_sprites/MXYLgFEcagg_texs_0.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_sprites/LKJLXbiOvBg_texs_0.jpg} \\


\multicolumn{4}{c}{CoDeF}\\
\includegraphics[width = 1.5in]{figures/sup_other_comp_codef/canonical_1_mic.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_codef/canonical_1_uncle.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_codef/canonical_1_green.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_codef/canonical_1_hand.png} \\

\includegraphics[width = 1.5in]{figures/sup_other_comp_codef/canonical_0_mic.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_codef/canonical_0_uncle.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_codef/canonical_0_green.png} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_codef/canonical_0_hand.png} \\

\multicolumn{4}{c}{Our \textit{VideoSPatS}}\\
\includegraphics[width = 1.5in]{figures/sup_other_comp_ours/e134_can_face_mic.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_ours/e120_can_face_uncle.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_ours/e120_can_face_green.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_ours/e134_can_face_hand.jpg} \\

\includegraphics[width = 1.5in]{figures/sup_other_comp_ours/e134_can_occ_mic.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_ours/e120_can_occ_uncle.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_ours/e120_can_occ_green.jpg} &
\includegraphics[width = 1.5in]{figures/sup_other_comp_ours/e134_can_occ_hand.jpg} \\

\end{tabular}

==> figures/super_other_comp_rec_backup.tex <==
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.6}
\small
\begin{tabular}{cccc}

\multicolumn{4}{c}{Neural Layered Atlases}\\
\includegraphics[width = 1.6in]{figures/sup_other_comp_atlasses/rec_mic.jpeg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_atlasses/rec_uncle.jpeg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_atlasses/rec_green.jpeg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_atlasses/rec_hands.jpeg} \\


\multicolumn{4}{c}{Deformable Sprites}\\
\includegraphics[width = 1.6in]{figures/sup_other_comp_sprites/Yu5Xu2qwZxo_recons_0.jpg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_sprites/C6VbIdO42mQ_recons_0.jpg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_sprites/MXYLgFEcagg_recons_0.jpg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_sprites/LKJLXbiOvBg_recons_0.jpg} \\

\multicolumn{4}{c}{CoDeF}\\
\includegraphics[width = 1.6in]{figures/sup_other_comp_codef/00049_mic.png} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_codef/00000_uncle.png} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_codef/00000_green.png} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_codef/00049_hand.png} \\

\multicolumn{4}{c}{Our \textit{VideoSPatS}}\\
\includegraphics[width = 1.6in]{figures/sup_other_comp_ours/e134_comp_img_mic.jpg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_ours/e120_comp_img_uncle.jpg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_ours/e120_comp_img_green.jpg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_ours/e134_comp_img_hand.jpg}  \\

\multicolumn{4}{c}{GT}\\
\includegraphics[width = 1.6in]{figures/sup_other_comp_gt/mic.jpg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_gt/uncle.jpg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_gt/green.jpg} &
\includegraphics[width = 1.6in]{figures/sup_other_comp_gt/hands.jpg} \\



\end{tabular}

==> notation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% CUSTOM COMMANDS START %%%%%%%%%%%%%%%%%%%%%%%%

\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\crefname{table}{Tab.}{Tabs.}
\Crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Figure}{Figures}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Equation}{Equations}
\hyphenpenalty=1200


% Network Names

% Voxel generator
\newcommand{\G}{\mathsf{G}}
% Camera predictor
\newcommand{\C}{\mathsf{C}}

% Volume
\newcommand{\V}{V}
% V^Density
\newcommand{\Vdens}{\V^{\mathrm{Density}}}
% V^Feat
\newcommand{\Vfeat}{\V^{\mathrm{RGB}}}
% V^LBS
\newcommand{\VLBS}{\V^{\mathrm{LBS}}}
% Frame
\newcommand{\f}{F}
% Occupancy
\newcommand{\occ}{O}
% Camera
\newcommand{\T}{T}
% Camera part
\newcommand{\Tp}{T_p}
% Rotation 
\newcommand{\rot}{R}
% Camera part
\newcommand{\rotp}{R_p}
% Translation
\newcommand{\tra}{t}
% Translation part
\newcommand{\trp}{t_p}
% Keypoints 3D
\newcommand{\kpthree}{K^{3D}}
% Keypoints 2D
\newcommand{\kptwo}{K^{2D}}
% Number of keypoints
\newcommand{\nk}{N_k}

% Video id
\newcommand{\id}{\alpha}
% Number of frames
\newcommand{\nf}{N_f}
% Number of features
\newcommand{\nfeat}{N_{feat}}
% Embedding size
\newcommand{\nemb}{N_e}
% Embedding
\newcommand{\emb}{\mathbf{e}}
% Part
\newcommand{\partidx}{p}
% Num Parts
\newcommand{\np}{N_p}
% Voxel size
\newcommand{\voxsize}{S}

% Codes for shape and pose for metrics computation
\newcommand{\yaw}{\Theta}
\newcommand{\shapecode}{c^s}
\newcommand{\posecode}{c^p}
% Num Parts
\newcommand{\shapecodelen}{N_{\shapecode}}
\newcommand{\posecodelen}{N_{\posecode}}

\newcommand{\secpostvspace}{\vspace{-0.05cm}}
\newcommand{\secprevspace}{\vspace{-0.05cm}}

\newcommand{\apppostvspace}{\vspace{-0.2cm}}
\newcommand{\appprevspace}{\vspace{-0.2cm}}
% Math
%Real
% \newcommand{\R}{\mathbb{R}}
% Natural
\newcommand{\N}{\mathbb{N}}

\newcommand{\projname}{3D-VADER}

\usepackage{xspace}

% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

% \newcommand{\eg}{\emph{e.g}\onedot}
% \newcommand{\Eg}{\emph{E.g}\onedot}
% \newcommand{\ie}{\emph{i.e}\onedot}
% \newcommand{\Ie}{\emph{I.e}\onedot}
%% \newcommand{\cf}{\emph{cf}\onedot}
%% \newcommand{\Cf}{\emph{Cf}\onedot}
%% \newcommand{\etc}{\emph{etc}\onedot}
% \newcommand{\vs}{\emph{vs}\onedot}
%% \newcommand{\wrt}{w.r.t\onedot}
%% \newcommand{\dof}{d.o.f\onedot}
%% \newcommand{\iid}{i.i.d\onedot}
%% \newcommand{\wolog}{w.l.o.g\onedot}
%% \newcommand{\etal}{\emph{et al}\onedot}

% \DeclareMathOperator{\E}{\mathbb{E}}
\newcommand{\vect}{\vec}
\newcommand{\stopgrad}{sg}

%%%%% bold symbols %%%%%%%%%%%
%%% used in the nerf %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% CUSTOM COMMANDS END %%%%%%%%%%%%%%%%%%%%%%%%


==> tables/davis_comp.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcccccc}
\hline
Scene & Neural Atlases~\cite{kasten2021layered} & CoDeF~\cite{ouyang2024codef} & \TODO{Ours} \\ 
\hline
Blackswan & 29.92 & 31.97 & \\
Boat      & 31.51 & 34.13 & \\
Kite-surf & 28.37 & 34.26 & \\

\hline
\end{tabular}

